Attentive Graph-based Text-aware Preference Modeling for Top-N Recommendation

Textual data are commonly used as auxiliary information for modeling user preference nowadays. While many prior works utilize user reviews for rating prediction, few focus on top-N recommendation, and even few try to incorporate item textual contents such as title and description. Though delivering promising performance for rating prediction, we empirically find that many review-based models cannot perform comparably well on top-N recommendation. Also, user reviews are not available in some recommendation scenarios, while item textual contents are more prevalent. On the other hand, recent graph convolutional network (GCN) based models demonstrate state-of-the-art performance for top-N recommendation. Thus, in this work, we aim to further improve top-N recommendation by effectively modeling both item textual content and high-order connectivity in user-item graph. We propose a new model named Attentive Graph-based Text-aware Recommendation Model (AGTM). Extensive experiments are provided to justify the rationality and effectiveness of our model design.

==> 4_related_work.tex <==
\section{Related Work}
% In this section, we review existing works that incorporate textual information into recommendation.

\subsection{Recommendation with KG}
Applying knowledge graph as auxiliary information to improve recommendation performance is a very common approach. Early works such as CKE~\cite{CKE} and KTUP~\cite{KTUP} apply KG embedding methods like TransE~\cite{TransE} and TransH~\cite{TransH} to learn entity embeddings, and use them as item information to guide the representation learning for recommendation. Later on, inspired by recently emerged graph convolutional network (GCN)~\cite{GCN} and other graph neural networks~\cite{GraphSAGE, GAT}, methods such as KGAT~\cite{KGAT}, CKAN~\cite{CKAN}, and KGIN~\cite{KGIN} apply embedding propagation schemes to model high-hop neighborhood information in user-item interaction graph and KG in order to capture more useful information into the final representations.

While having some common ideas, our work differs from those models fundamentally. Those works utilize KG triples, which is a structured data, while our task is to model unstructured textual information. Furthermore, we devised a new propagation scheme that models user preference solely based on item textual representation, which is a totally unseen approach.

\subsection{Review-Based Recommendation}
There are a thread of works that incorporate review texts into recommendation models. An early work named DeepCoNN~\cite{DeepCoNN} represents a user as all the reviews they have written, and an item as all the reviews it has received. The user and item documents are then encoded by convolutional neural networks (CNNs) and passed into a Factorization Machine (FM)~\cite{FM} for prediction. Later methods apply a similar paradigm~\cite{TransNets, Dattn, NARRE, MPCN} with some changes such as modeling reviews independently~\cite{NARRE, MPCN}.

Although those works also model textual information, they all focus on rating-based prediction, which is to predict the rating to an item for a user, instead of top-N personalized recommendation. Also, the item textual contents are generally better in quality and reliability than user reviews. They provide a more specific and accurate information for items, which is a reason why we focus on adopting item textual content as auxiliary information for recommendation. 

\subsection{Clicked-Based News Recommendation}
There are a series of works specifically focus on news recommendation.  Traditional methods rely on manual feature engineering to build user and news (item) representations, such as Wide \& Deep~\cite{WnD}, DeepFM~\cite{DeepFM}, and NFM~\cite{NFM}. Later works start to use neural networks to learn user and news representations directly, such as DKN~\cite{DKN} and NPA~\cite{NPA}. Some following works~\cite{LSTUR, NAML, NRMS} apply attention networks on news representations and learn user representations by aggregating clicked news by users. Inspired by the recent advances of pretrained Transformer-based language models, recent works such as RMBERT~\cite{RMBERT} and UNBERT~\cite{UNBERT} leverage the ability of content modeling from BERT~\cite{BERT} to extract news representation.

Different from the news recommendation task, we focus on top-N personalized recommendation, while news recommendation models focus on click prediction. Furthermore, to our best knowledge, none of those methods apply GCN to model high-hop neighborhood information.

